Mobile Networks on the Move: Optimizing Moving Base Stations Dynamics in Urban Scenarios

Base station densification is one of the key approaches for delivering high capacity in radio access networks. However, current static deployments are often impractical and financially unsustainable, as they increase both capital and operational expenditures of the network. An alternative paradigm is the moving base stations (MBSs) approach, by which part of base stations are installed on vehicles. However, to the best of our knowledge, it is still unclear if and up to which point MBSs allow decreasing the number of static base stations (BSs) deployed in urban settings. In this work, we start tackling this issue by proposing a modeling approach for a first-order evaluation of potential infrastructure savings enabled by the MBSs paradigm. Starting from a set of stochastic geometry results, and a traffic demand profile over time, we formulate an optimization problem for the derivation of the optimal combination of moving and static BSs which minimizes the overall amount of BSs deployed, while guaranteeing a target mean QoS for users. Initial results on a two-district scenario with measurement-based network traffic profiles suggest that substantial infrastructure savings are achievable. We show that these results are robust against different values of user density.

==> 00_abstract_OLD.tex <==
\begin{abstract} 
Base station densification is one of the key approaches for the delivery of high capacity in radio access networks. However, current static deployments are often impractical and financially unsustainable, as it increases both capital (CAPEX) and operational (OPEX) expenditures of the network. An alternative paradigm is the moving base stations (MBS) approach, by which part of base stations are installed on vehicles, giving rise to an emergent "natural densification" behavior. However, to the best of our knowledge, it is still unclear if and up to which point MBSs actually allow decreasing the number of static base stations (BS) deployed in urban settings.
In this work, we start tackling this issue by proposing a modeling approach for a first-order evaluation of potential infrastructure savings enabled by the MBS paradigm. Starting from a set of stochastic geometry results, and a traffic demand profile over time, we formulate an optimization problem for the derivation of the optimal combination of moving and static BS which minimizes the overall amount of BS deployed, while guaranteeing a target mean QoS for users. Our approach takes as input realistic patterns of traffic demand for each district of an urban scenario and a given time interval, and it derives the overall amount of static infrastructure required in each district, as well as the overall amount of MBS sufficient to satisfy the traffic demand. Initial results on a two-district scenario with measurement-based network traffic profiles suggest that substantial infrastructure savings are indeed achievable. We show that these results are robust against several key system parameters and different user densities.
\end{abstract}

==> 01_Intro_OLD.tex <==
\section{Introduction}

Cellular networks will face significant technical and economic challenges soon, primarily driven by the escalating number of users and the growing demand for data traffic, especially in urban settings. According to the forecasting analysis in \cite{forecast}, in future systems the per-area data volume will increase by 1000 times, while the number of connected devices and the user data rate will increase by 10 to 100 times. To address this challenge, network densification, which was already exploited in 5G \cite{densification}, was proposed. However, this approach leads to an increase in both capital expenditure (CAPEX) and operational expenditure (OPEX) of the network. Furthermore, densification is strictly related to over-provisioning, i.e. worst-case dimensioning and deployment of network resources, to cope with traffic peaks and with the increasing variability of traffic over time. To reduce network costs and installations, other solutions have been explored. One approach is the deployment of small cells or Distributed Antenna Systems (DAS). Among all of them, a promising alternative lies in the dynamic mobile network paradigm \cite{dymonetproposal}. The moving small cell base stations (BSs) provide additional capacity, when and where needed, to the end users of an otherwise traditional RAN. End-user terminals can thus freely and transparently transfer their services between a normal and a vehicular BS. Studies about the optimal positioning and other challenges related to the mobility of MBSs have already been investigated and solved as in \cite{optimalpos}. Existing studies confirm the adaptability of MBSs, which have the potential to align with both spatial and temporal variations in the number of mobile users and the level of traffic they generate in urban scenarios \cite{AJMONEMobilenet}. However, to the best of our knowledge, nobody has quantified, if existing, the possible reduction in densification that could result from the introduction of MBSs. We aim to provide a framework to evaluate the potential CAPEX savings when using MBSs.
In this paper, we develop an approach for determining the optimal number of mobile BS required to implement a hybrid network, i.e., that encompasses both fixed and mobile BS, where the CAPEX is lower than in a traditional cellular network. The optimal solution represents the right balance of moving and static BS, minimizing the total number of installed BS while guaranteeing the desired Quality of Service (QoS) for all users. Our study can be applied either to design an entirely new cellular network or, more realistically, to enhance the service in a certain area while avoiding network densification. If we have an esteem of future traffic in a certain area, where some static BS (SBSs) are already in place, we can determine the optimal number of static and moving BS to add in the specific scenario to meet the increased demand for connectivity.
Our main contributions are:
\vspace{-0.1in}
\begin{itemize}
    \item We formulate a linear optimization problem to determine the optimal number of moving and static BS required in a given scenario to serve a given traffic demand with a target QoS;
    \item We propose an approach to compute CAPEX savings, which is based on the forecasted patterns of traffic demand in each district of an urban scenario for a given time interval. By solving the optimization problem, it computes the overall amount of static infrastructure required in each district (with and without MBS), as well as the overall minimum amount of MBS which allows satisfying the traffic demand in the whole city for the given time interval. 
    %We propose a method to compute the baseline for installed static base stations in our modeled urban scenario. This baseline is then exploited to assess the savings in CAPEX through an optimization problem;
    \item We apply our approach on a two-district scenario, for a first-order evaluation of the savings achievable with the MBS paradigm. Results suggest that MBS enables substantial savings (reaching a maximum of $21\%$ in the considered settings) in the total amount of deployed BS. We show that these results are robust with respect to different values of mean user density in each district.
\end{itemize}

==> 04_numerical_results_OLD.tex <==
\section{Numerical Results}
\label{numerical results}


In this section, we validate numerically our approach. We consider an ideal, simplified urban scenario, composed of two regions with different patterns of network traffic demand. Namely, the first region models a residential area, and the second one models a business and office area. The daily network traffic profiles of the two areas are derived from operator data~\cite{9448695}, and they are shown in Fig. \ref{comparisons}a. Note that the peak in traffic of a region happens roughly at the same time at which there is a low in traffic in the other region. This suggests that a substantial amount of MBSs could be reused by moving them over time from one region to the other, to cater for peaks in traffic demand.  
%\subsection{System setup}
 We partition the $24h$ observation window into 
 $60$ equal-sized intervals.
We consider a target mean throughput of $100$ kbps (e.g., the data rate requested by a Skype call), which corresponds to a per-bit delay of $10^{-5} \frac{s}{bit}$. 
Base stations work at a frequency of $1$ GHz and use a bandwidth of $10$ MHz.
We assume that BS and MBS have the same energy consumption. 
%This is not necessarily true since MBS need a battery to charge them and wireless backhauling \cite{MBSconsumption}. \\
To estimate the mean number of active network users in every region, the network traffic profiles have been normalized and rescaled in such a way as to have the peak of active user density coincide with values that are considered reasonable in future dense urban scenarios \cite{worldpopulationreviewMilanPopulation}. Specifically, we set it to $10000$ and $1000$ people per $km^2$ for the business and residential districts respectively. 
%Thus, the ratio between the densities in the office region and R is 10. 
Unless otherwise stated, we assumed a ratio between the areas of the office and residential regions (henceforth denoted as \textit{area ratio}) of $10$. We have considered scenarios in which the residential area is always larger than the office area, as is common in 
many urban settings.
We have considered an office area of 1 $km^2$. Thus, an area ratio of one corresponds to a residential region of 1 $km^2$ too.

\vspace{-0.1in}
\subsection{Evaluation}

\begin{figure*}[ht!]
     \centering
     \subfloat[\centering Traffic profiles]{\includegraphics[width=.3\linewidth]{figures/profiles.eps}}
      \subfloat[\centering Office district]{ \includegraphics[width=.3\linewidth]{figures/officecomplete.eps}}
        \subfloat[\centering Residential district]{\includegraphics[width=.3\linewidth]{figures/residencecomplete.eps}}
        
        %\subfloat[\centering $|V| = 24 $]{\includegraphics[width=.23\textwidth]{figures/mnist_24_0.1.png}} \\
         %\subfloat[\centering $|V| = 24$]{\includegraphics[width=.23\textwidth]{figures/mnist_24_1.png}}
%      \caption{Mean accuracy versus round for \ac{OGL}, random GL, and DP algorithm using the MNIST dataset.}  
%      \label{fig:mnist_comparisons}
%      \vspace{-15pt}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[ht!]
%      \centering
   
     \caption{(a) Normalized daily mobile traffic profiles in the resident (red) and office (blue) district; (b), (c): Optimal number of MBS (green), total number of BS (orange) with respect to the baseline (red), and installed BS in the static scenario (black) for the two regions over 24 hours. The total number of active base stations over the all area is given by the superposition of the orange dashed lines in the 2 plots.}  
     \label{comparisons}
     \vspace{-15pt}
\end{figure*}

\begin{figure*}[ht!]
     \centering
        \subfloat[]{\includegraphics[width=.3\linewidth]{figures/PercMBSR.eps}}
       \subfloat[]{\includegraphics[width=.3\linewidth]{figures/bothratios.eps}}
      \subfloat[]{\includegraphics[width=.3\linewidth]{figures/costsavingwithratio.eps}}
        
        %\subfloat[\centering $|V| = 24 $]{\includegraphics[width=.23\textwidth]{figures/mnist_24_0.1.png}} \\
         %\subfloat[\centering $|V| = 24$]{\includegraphics[width=.23\textwidth]{figures/mnist_24_1.png}}
%      \caption{Mean accuracy versus round for \ac{OGL}, random GL, and DP algorithm using the MNIST dataset.}  
%      \label{fig:mnist_comparisons}
%      \vspace{-15pt}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[ht!]
%      \centering
   
     \caption{(a) Fraction of the total amount of MBS in the scenario allocated to the residential area, over the $24$ hours; (b) Saving with respect to the fully static scenario, in terms of installed SBS in the residential and office districts and in terms of both moving and static BS in the whole area, as a function of the ratio between the values of maximum density of connected users in the two regions; (c) Cost saving with respect to the fully static scenario, as a function of the ratio between the unitary cost of static BSs, and that of moving BSs. }  
     \label{analysis}
     \vspace{-15pt}
\end{figure*}

 
%Our first step consists of solving the problem in \ref{prob:0} to obtain the optimal number of active static BS $\lambda_{b,j}^z$ over each hour of the day, for each region, considering that the density of users connected to the network varies according to the adopted traffic profiles. 
%In the following steps, we use these optimal density values as input parameters for the constraints of the optimization problem in \ref{prob:1}. 

In a first set of experiments, we have derived the optimal number of MBS in every time slot and the optimal total number of BS in both regions, as derived from the solution of Problem 2, as well as the minimum number of BS required to serve users in each region with the given target QoS, over 24 hours, as derived from the solution of Problem 1 (denoted as the "baseline"). As Fig. \ref{comparisons} shows,  %the optimal number of MBS and the optimal total number of BS in both regions, as derived from the solution of Problem 2, as well as the minimum number of BS required to serve users in each region with the given target QoS, over 24 hours, as derived from the solution of Problem 1 (denoted as the "baseline"). 
%For the sake of completeness, the plots also include the values for $\lambda_{b,j}^z$. 
%The maximum number of BS we need to install to serve all users over the day, without MBS, corresponds to the maximum of these values in each area.
 %even if the density of connected users is lower in the residential region, we need more BS installed than in the office region. Specifically, for the chosen values, in the office region, there are $33\%$ less BS than in the residential region. 
 the optimal density of \textit{active} BSs (baseline curve in Fig. 1b and 1c) is roughly directly proportional to the density of active users. The maximum of this quantity in each region (straight black line in Fig. 1b and 1c) is the number of BSs installed in the purely static scenario. Being dimensioned for peak traffic, the static scenario is vastly redundant during the majority of the day, with important implications in terms of consumed power. The plots show also how the adaptive densification brought in by MBSs substantially reduces the amount of redundant infrastructure during the 24h, reducing energy consumption and the need for dynamic power management in both regions. The plots show also that the maximum aggregate traffic demand in the two regions over the day (taking place at around $10$ AM in our experiments) ultimately determines the overall amount of static and moving BS deployed in the whole scenario. As a consequence of the fact that the overall number of MBS is driven by peak aggregate traffic demand, some amount of overprovisioning is present also in the population of MBS. This is visible in Fig 1, in which the amount of off-peak total BS density is almost always above the minimum required to serve users. In realistic settings, this extra service capacity is however useful to account e.g., for a weak correlation between patterns of densification in the population of vehicles in the two regions, and patterns of network traffic demand. On the other hand, our evaluation of the number of base stations in excess  allows estimating the potential for energy savings achievable by adapting, in each time slot, the number of active (i.e. not in standby mode, and ready to serve users) base stations in each area, to have it coincide with the minimum required to serve users with the target QoS.\\  
Fig. 2a shows how the population of MBS is shared between the two regions at the optimum, as a function of the time of the day. The figure suggests that MBS are shared in an approximately equal manner between the two regions for most of the day. However, in the period during which network traffic demand peaks in the residential area, almost all of the MBSs converge there to supply the service capacity required. This strongly correlates with typical traffic patterns in an urban scenario, and further supports the feasibility of the moving base station paradigm in these settings.\\
%Assuming the implementation of a sleep strategy for both static and moving base stations, the system can effectively switch off unnecessary BS during periods of inactivity to save energy.
One of the key system parameters that determine the optimal deployment strategies resulting from our approach is the density of connected users over the observation window. To make our results more robust, in a new set of experiments, we evaluated how the savings in the total amount of BS deployed enabled by the moving base station paradigm are impacted by this parameter. Specifically, we conduct our analysis by varying the ratio between the maximum density of connected users in the office district and the same quantity for the residential district (henceforth denoted as \textit{user density ratio}) while keeping constant the total number of users during peak hours. To achieve this, we adjust the area ratio.
Assuming a profile of total number of active network users in the office district equal to the one in Figure 1a, we set the peak at 10.000 users per square kilometer. Then we tuned the user density ratio letting the maximum density of connected users in the residential district vary. We assumed the total number of active users, in both regions, as a function of time to be the same as in Fig. 1a. This allows us to check the impact of different active user densities, but more importantly, of different ratios between the density of active users in the office and residential regions. As such densities are key in determining the minimum density of BS that allows serving users with the target QoS, such an experiment is crucial to test the robustness of our results. Results relative to a user density ratio ranging from 1 to 10 can be found in Figure \ref{analysis}b and show a decrease of the total amount of base stations deployed (mobile and static) of $17\%$ on average in all configurations and all areas, with respect to the fully static configuration, and up to $21\%$ for low values of user density ratio. Thus, the moving base stations paradigm, coupled with optimal MBS deployment strategies, proves able to achieve the target user-perceived QoS while substantially decreasing the amount of static BS deployed, over a large spectrum of configurations in terms of area ratio.
In addition, the reduction in the amount of \textit{static} BS deployed with respect to the static configuration varies between $95\%$ for low user density ratios, to $70\%$ for higher values. As expected, such a decrease is inferior with a larger user density ratio. Indeed, 
larger values of this parameter imply that residential active users are spread over a larger area, with on average, a larger mean distance from the serving base station.
This brings as a consequence a decrease in the efficiency of the information transfer, thus an increase of the mean amount of base stations required to serve users, even in periods of low network traffic demand. As a consequence, we witnessed a reduction in the margins for MBS reuse in the two regions, and thus in the gains of the moving base stations paradigm. Anyway, the overall results show that MBS can remarkably decrease the dependence of the network on static deployments, which typically imply higher costs and must account for way tighter administrative and legal constraints than for MBS.\\
%Note that the percentage decrease in static BS deployed, as per Figure \ref{analysis} a, is not monotonic with respect to the area ratio. This is due to the fact that, by varying the area ratio,
%Additionally, on average, 72\% of the base stations are moving. 
%%%%%%%%%%%%%%%%%
%\subsection{Area ratio}
%The relative dimension of the areas is one of the main parameters of our model, since it affects the overall amount of MBS which have to be deployed. 
%In a new set of experiments, we varied the ratio between the areas of the two regions, while assuming that the office area is always smaller than the residential area. Furthermore, we kept the density in the office region static because the algorithm that finds the optimal number of BS is nonlinear and depends sensibly on users' density.
%As key performance indicators (KPIs) for our analysis, we chose the following: the percentage of total moving base stations compared to the total number of BS at the optimum;the CAPEX savings in terms of static BS installation at the optimum compared to the theoretical number of BS required to serve all users within the two specified areas; the overall CAPEX savings, taking into account both moving and static installed BS, with respect to the baseline.
%\subsection{Relative cost of static and moving BS}
Finally, we have considered 
 a variation of Problem 2, in which static and moving BS have different unitary costs, and we have 
 evaluated the impact of the ratio between the unitary costs of the two types of BSs on the overall amount of savings achievable with respect to purely static deployments.
Note that our assumption in this analysis is that moving and static base stations share the same energy consumption, and therefore, we do not consider operational expenditure (OPEX) savings.
% In the existing literature, few studies are addressing the absolute costs of BS, many of them adopt values from the work in \cite{bscostsource}. However, it's crucial to note that this source is outdated, and the costs of base stations have shown considerable variability over time and space. To offer a more comprehensive analysis, we decided to examine the ratio between the cost of a static BS and moving BS, thereby ensuring that the results are not dependent on specific values. 
In particular, we have assumed that SBSs have a higher unitary cost than MBSs. This is primarily because static base stations typically require larger HW modules, and higher installation costs (including, e.g. rental of the roof area). 
As Fig. \ref{analysis}c shows, when the cost of static base stations rises compared to the cost of moving base stations, the optimal configuration implies a larger fraction of moving BSs. In this scenario, the system tends to use MBS not only due to their ability to commute between the two areas, facilitating reuse, but also because they are cheaper. 
%As illustrated in the plot, the maximum number of MBS that the system can utilize depends on the number of MBS needed to cover the largest gap between the various traffic demands. For the selected traffic profiles, this gap corresponds to the latest hours of the day when users concentrate in the residential district.

==> blank.tex <==
The total network traffic in the two areas during peaks is the same, but we need more BS to satisfy the demanded QoS in the residential region because the model takes into account that residential users are on average more distant from their serving BS. Thus, it is necessary to activate more BS to guarantee the target QoS. 


\textbf{This preliminary evaluation suggests that the concept of dynamic mobile networks can substantially reduce the number of BS to install.
}
As the plots suggest, in each region there is a time of the day when the optimal number of base stations matches the minimum number sufficient to guarantee the target QoS, and thus where the performance constraints in Problem 2 are tight. As this happens only once in each region, these times of the day are thus those in which the dimensioning drives the overall amount of infrastructure required to serve users in the considered scenario.

==> common/new_commands.tex <==

% % how to change Contents to Table of Contents
% \addto\captionsenglish{% Replace "english" with the language you use
%   \renewcommand{\contentsname}%
%     {Table of Contents}%
% }

% to change the name of Abbreviations to Acronyms
% not needed if use use entry types and define those
% \renewcommand{\abbreviationsname}{Acronyms}

% to allow line comments in algorithms
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}

% to declare abs and norm
\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\norm{\lVert}{\rVert}%

% Swap the definition of \abs* and \norm*, so that \abs
% and \norm resizes the size of the brackets, and the 
% starred version does not.
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
%
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\makeatother



==> common/package_config.tex <==
% configuration for glossaries
% convert and load converted glossaries in .tex ,format from .bib
\setabbreviationstyle{long-short-desc} % style before loading resources
% this command sets the style to title for long names of acronyms only in the glossary description, leading to capitalized first-letter for all words
% \glssetcategoryattribute{\glsxtrabbrvtype}{glossname}{capitalisewords} % doesn't work
% resources to load if using a bib file with bib2gls
%\GlsXtrLoadResources[%
% src={glossaries}, % name of the file without extension
% selection=all, % select all the entries
%]
% not needed
%\newglossary*{abbreviation}{Acronyms} % to change the name of this glossary for acronyms

%\renewcommand{\glsclearpage}{\paginavuota} % to allow glossaries to clear pages, done manually is better


% setup for hyperref
\hypersetup{%
    pdfpagemode={UseOutlines},
    bookmarksopen,
    pdfstartview={FitH},
    colorlinks,
    linkcolor={black}, % it is suggested to keep them black, since when printing it it costs per page, and if they have color it's twice the price per page
    citecolor={black},
    urlcolor={black}
  }
%

% setup for svg
\svgsetup{%
    inkscapeformat=pdf, % to force usage of PDF
    inkscapelatex=false, % to disable latex rendering of text, produces errors
}

% setup for siunitx, it does not work in the summary
\sisetup{%
    detect-all, % to use the same font as for writing when using \num
    mode=text, % to allow it to work also in math mode
    group-separator = {,}, % separator for number grouping
    group-minimum-digits = 3, % minimum number of digits a number must have to be grouped in 3-digit groups
}

% listings colours
\definecolor{rulecolor}{rgb}{0,0,0}
\definecolor{commentcolor}{rgb}{0,0.6,0}
\definecolor{linenumbercolor}{rgb}{0.5,0.5,0.5}
\definecolor{keywordcolor}{rgb}{0,0,0.95}
\definecolor{backcolor}{rgb}{1,1,1}%{0.95,0.95,0.92}
\definecolor{stringcolor}{rgb}{0.58,0,0.82}

% setup for lstlisting
\lstset{ %
	backgroundcolor=\color{backcolor},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
	basicstyle=\footnotesize,        % the size of the fonts that are used for the code
	breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
	breaklines=true,                 % sets automatic line breaking
	captionpos=t,                    % sets the caption-position to bottom
	commentstyle=\color{commentcolor},    % comment style
	extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
	frame=single,	                   % adds a frame around the code
	keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
	keywordstyle=\color{keywordcolor},       % keyword style
	%language=VHDL,                 % the language of the code
	numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
	numbersep=5pt,                   % how far the line-numbers are from the code
	numberstyle=\tiny\color{linenumbercolor}, % the style that is used for the line-numbers
	rulecolor=\color{rulecolor},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
	showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
	showstringspaces=false,          % underline spaces within strings only
	showtabs=false,                  % show tabs within strings adding particular underscores
	stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
	stringstyle=\color{stringcolor},     % string literal style
	tabsize=4,	                   % sets default tabsize to 2 spaces
	title=\lstname,                   % show the filename of files included with \lstinputlisting; also try caption instead of title
	inputencoding=utf8,
	literate=
	{á}{{\'a}}1 {é}{{\'e}}1 {í}{{\'i}}1 {ó}{{\'o}}1 {ú}{{\'u}}1
	{Á}{{\'A}}1 {É}{{\'E}}1 {Í}{{\'I}}1 {Ó}{{\'O}}1 {Ú}{{\'U}}1
	{à}{{\`a}}1 {è}{{\`e}}1 {ì}{{\`i}}1 {ò}{{\`o}}1 {ù}{{\`u}}1
	{À}{{\`A}}1 {È}{{\'E}}1 {Ì}{{\`I}}1 {Ò}{{\`O}}1 {Ù}{{\`U}}1
	{ä}{{\"a}}1 {ë}{{\"e}}1 {ï}{{\"i}}1 {ö}{{\"o}}1 {ü}{{\"u}}1
	{Ä}{{\"A}}1 {Ë}{{\"E}}1 {Ï}{{\"I}}1 {Ö}{{\"O}}1 {Ü}{{\"U}}1
	{â}{{\^a}}1 {ê}{{\^e}}1 {î}{{\^i}}1 {ô}{{\^o}}1 {û}{{\^u}}1
	{Â}{{\^A}}1 {Ê}{{\^E}}1 {Î}{{\^I}}1 {Ô}{{\^O}}1 {Û}{{\^U}}1
	{œ}{{\oe}}1 {Œ}{{\OE}}1 {æ}{{\ae}}1 {Æ}{{\AE}}1 {ß}{{\ss}}1
	{ű}{{\H{u}}}1 {Ű}{{\H{U}}}1 {ő}{{\H{o}}}1 {Ő}{{\H{O}}}1
	{ç}{{\c c}}1 {Ç}{{\c C}}1 {ø}{{\o}}1 {å}{{\r a}}1 {Å}{{\r A}}1
	{€}{{\euro}}1 {£}{{\pounds}}1 {«}{{\guillemotleft}}1
	{»}{{\guillemotright}}1 {ñ}{{\~n}}1 {Ñ}{{\~N}}1 {¿}{{?`}}1
}


% % biblatex setup
% % generally 9000 is ok, if higher than 10000 it's bad
% % If you want to break on URL numbers
% \setcounter{biburlnumpenalty}{9000}
% % If you want to break on URL lower case letters
% \setcounter{biburllcpenalty}{9000}
% % If you want to break on URL UPPER CASE letters
% \setcounter{biburlucpenalty}{9000}


==> misc_old/05_parameter_analysis.tex <==
% \section{Parameters analysis}
% \label{param_analysis}
One of the key system parameters that determine the optimal deployment strategies resulting from our approach is the area ratio. In a new set of experiments, we evaluated how the savings in the total amount of BS deployed enabled by the moving base station paradigm are impacted by the area ratio.
Figure \ref{analysis} shows the decrease in the total amount of static BS deployed, in the two considered regions, with respect to the configuration without MBS. The plots show that the moving base stations paradigm, coupled with optimal MBS deployment strategies allows achieving the given target user-perceived QoS while decreasing the amount of static BS deployed by at least $70\%$. As expected, such a decrease is inferior with a larger area ratio. Indeed, 
larger values of this parameter imply that users in the residential district are distributed over a wider area, and they are thus on average more distant from their respective serving base stations. This implies a lower efficiency in the delivery of information to users on behalf of the network, and thus the need for larger BS densities to deliver the same target QoS to users.\\ 
\com{Note that the percentage decrease in static BS deployed, as per Figure \ref{analysis}, is not monotonic with respect to the area ratio. This is due to the fact that, by varying the area ratio,
we also change the total amount of MBS required to serve users in the whole scenario, at the optimum. And this latter quantity does not vary monotonically with the area ratio, as it depends also crucially on the.... 
EXPLAIN OR KILL 
To assess the robustness of our results, we analyzed the mean ($\mu$) and standard deviation ($\sigma$) of our distributions. Specifically, we compute the coefficient of variation, $CV = \frac{\sigma}{\mu}$ to provide insight into the extent of the spread of values in the residential region in relation to the average.
Given that, for each distribution, the computed coefficient of variation is less than $0.2$, we can conclude that, even when altering the ratio between the two areas, an average decrease of static BS deployments in the office region of $43\%$ is achievable. }


%Additionally, on average, 72\% of the base stations are moving. 
%%%%%%%%%%%%%%%%%


we evaluated different ratios of the residential and office areas and concluded that incorporating MBS always results in a reduction of the overall amount of deployed BS.
In another set of experiments, we considered different unitary costs for MBS and static BS, eg. due to differences in installation and bureaucratic expenses. As Fig 2 shows, as the relative cost of static BS increases, so does the overall cost of the BS deployments at the optimum, and the relative amount of MBS of the optimal configurations. However, for a relative cost larger than 2 the amount of savings stabilizes. 

%\subsection{Area ratio}


The relative dimension of the areas is one of the main parameters of our model, since it affects the overall amount of MBS which have to be deployed. 
In a new set of experiments, we varied the ratio between the areas of the two regions, while assuming that the office area is always smaller than the residential area. Furthermore, we kept the density in the office region static because the algorithm that finds the optimal number of BS is nonlinear and depends sensibly on users' density.
As key performance indicators (KPIs) for our analysis, we chose the following: the percentage of total moving base stations compared to the total number of BS at the optimum;the CAPEX savings in terms of static BS installation at the optimum compared to the theoretical number of BS required to serve all users within the two specified areas; the overall CAPEX savings, taking into account both moving and static installed BS, with respect to the baseline.

\com{To clarify the variability in the KPIs, we investigated the \textit{outlier points} and compared them with points closer to the average.
Our analysis reveals that, for those specific values of $\rho$, the optimal number of static and moving BS in the residential district exceeds the baseline and the system needs more static BS than in the other scenarios. Furthermore, in the business district, the optimal number of static BS is sufficient to meet the demand during certain time slots within the day, without the need for MBS. This accounts for the surplus of base stations on the residential side since the closted-system assumption holds true. 
Additionally, since the density of users, thus the number of BS required in the residential region, with respect to the analogous quantity in the office region, increases substantially as the ratio increases, the model can utilize fewer moving base stations to bridge the gap.}

As we expected, the savings in terms of installed BS is correlated with the amount of MBS introduced in the system: the more MBS we can exploit, the less BS we need to install. The versatility of moving base stations, that can be reused in the regions, allows savings in the two districts.

\subsection{Relative cost of static and moving BS}

This section examines how varying costs for moving and static base stations affect optimal base station density. 
It is important to note that our assumption in this analysis is that moving and static base stations share the same energy consumption, and therefore, we do not delve into operational expenditure (OPEX) savings.
In the existing literature, few studies are addressing the absolute costs of BS, many of them adopt values from the work in \cite{bscostsource}. However, it's crucial to note that this source is outdated, and the costs of base stations have shown considerable variability over time and space. To offer a more comprehensive analysis, we decided to examine the ratio between the cost of a static BS and moving BS, thereby ensuring that the results are not dependent on specific values. Specifically, we assume that SBSs have higher capital costs than MBSs. This is primarily because static base stations typically require more operations in terms of installation and permissions. We resume results from our analysis in figure \ref{analysis}. As we expected, when the cost of static base stations rises in comparison to the cost of moving base stations, the system tends to utilize more moving base stations to serve users. This trend is noticeable even when static BS costs less than 1.5 times that of moving BS. As a consequence, the average CAPEX savings, amounting to 48\%, is higher than the average CAPEX savings from the previous analysis. Specifically, in this scenario, the system tends to use MBS not only due to their ability to commute between the two areas, facilitating reuse but also because they are more cost-effective.
